RBF-Solver: A Multistep Sampler for Diffusion Probabilistic Models via Radial Basis Functions

Diffusion probabilistic models (DPMs) are widely adopted for their outstanding generative fidelity, yet their sampling is computationally demanding. Polynomial-based multistep samplers mitigate this cost by accelerating inference; however, despite their theoretical accuracy guarantees, they generate the sampling trajectory according to a predefined scheme, providing no flexibility for further optimization. To address this limitation, we propose RBF-Solver, a multistep diffusion sampler that interpolates model evaluations with Gaussian radial basis functions (RBFs). By leveraging learnable shape parameters in Gaussian RBFs, RBF-Solver explicitly follows optimal sampling trajectories. At first order, it reduces to the Euler method (DDIM). At second order or higher, as the shape parameters approach infinity, RBF-Solver converges to the Adams method, ensuring its compatibility with existing samplers. Owing to the locality of Gaussian RBFs, RBF-Solver maintains high image fidelity even at fourth order or higher, where previous samplers deteriorate. For unconditional generation, RBF-Solver consistently outperforms polynomial-based samplers in the high-NFE regime (NFE >= 15). On CIFAR-10 with the Score-SDE model, it achieves an FID of 2.87 with 15 function evaluations and further improves to 2.48 with 40 function evaluations. For conditional ImageNet 256 x 256 generation with the Guided Diffusion model at a guidance scale 8.0, substantial gains are achieved in the low-NFE range (5-10), yielding a 16.12-33.73% reduction in FID relative to polynomial-based samplers.

==> 5.Experiments/trajectory.tex <==
\subsection{Model Evaluation Trajectory}
\label{app:model_evaluation_trajectory}

Table~\ref{tab:traj_only} lists, for a 5-step schedule, the data evaluations produced by each solver and the relative magnitudes of the associated coefficients.  
Each coefficient multiplies either the current evaluation $\hat{\bm x}_\theta(\hat{\bm x}_{\lambda_{t_i}}, \lambda_{t_i})$ or the previous evaluation $\hat{\bm x}_\theta(\hat{\bm x}_{\lambda_{t_{i-1}}}, \lambda_{t_{i-1}})$.  
We take their absolute values and normalise them so that they sum to one.  
(See Appendix~\ref{app:Additional Details on Coefficient Computation} for a detailed description of how the coefficients are obtained for each solver.)

At low NFEs—such as five steps—the evaluation changes rapidly, and putting too much weight on the previous evaluation can reduce the quality of the final result.  
By optimising the shape parameter, RBF-Solver adaptively determines how much of the previous evaluation to reference, which helps produce higher-fidelity samples.

\begin{table*}[t]
  \centering
  \caption{Model evaluations and coefficient ratios. For each sampler, the table presents the model evaluations (data predictions) obtained at each of the five sampling steps, together with the relative magnitudes of the corresponding second-order coefficients.}
  \label{tab:traj_only}

  % 행 전체 높이도 약간 키움 (선택)
  \renewcommand{\arraystretch}{1.0}
  \setlength{\tabcolsep}{6pt}
  \begin{tabular}{M{0.18\linewidth} M{0.78\linewidth}}
    \toprule
    \textbf{Sampler} & \textbf{Model Evaluations and Coefficient Ratios} \\
    \midrule
    \addlinespace[4pt]
    \textbf{DPM-Solver++} &
    \includegraphics[width=\linewidth]{5.Experiments/trajectory/dpm_traj.png} \\
    \midrule
    \addlinespace[4pt]
    \textbf{UniPC} &
    \includegraphics[width=\linewidth]{5.Experiments/trajectory/unipc_traj.png} \\
    \midrule
    \addlinespace[4pt]
    \textbf{RBF-Solver} &
    \includegraphics[width=\linewidth]{5.Experiments/trajectory/rbf_traj.png} \\
    \bottomrule
  \end{tabular}
\end{table*}
